Algorithms for the Bin Packing Problem with Scenarios

This paper presents theoretical and practical results for the bin packing problem with scenarios, a generalization of the classical bin packing problem which considers the presence of uncertain scenarios, of which only one is realized. For this problem, we propose an absolute approximation algorithm whose ratio is bounded by the square root of the number of scenarios times the approximation ratio for an algorithm for the vector bin packing problem. We also show how an asymptotic polynomial-time approximation scheme is derived when the number of scenarios is constant. As a practical study of the problem, we present a branch-and-price algorithm to solve an exponential model and a variable neighborhood search heuristic. To speed up the convergence of the exact algorithm, we also consider lower bounds based on dual feasible functions. Results of these algorithms show the competence of the branch-and-price in obtaining optimal solutions for about 59% of the instances considered, while the combined heuristic and branch-and-price optimally solved 62% of the instances considered.

==> tex/old_aptas.tex <==
%
%Let $G_\calj$ be the subset of ``large'' items of $\calj$, i.e. $G_\calj = \{j
%\in \calj \mid s_j > \eps\}$, with~$\eps>0$ being a small constant. We denote
%$|G_\calj| = n_{G_\calj}$.
%%Consider a subset $G_\cali$ of $\cali$ with only large items, i.e. $G_\cali = \{i \mid s_i > \eps\}$. The amount of items of different sizes in $G_\cali$ is a constant, say $V$. There are $n_g$ large items in the instance, i.e. $|G_\cali| = n_g$.
%
%
%%An instance for the BPS Problem is a tuple $(I,n,\cals,d,s)$ such
%%that $I$ is a set of $n$ items, $\cals=\{S_1,\ldots,S_d\}$ is a set
%%of $d$ scenarios and $s_i>0$ is the weight of the item $i\in I$.
%%
%We denote by $\cali$ the set of all instances for the BPS Problem;
%%
%$\calg_{\eps}$ the set of instances in $\cali$ where all items have
%weight at least $\eps$;
%%
%$\cals$ the set of scenarios and $\cali_k$ the set of items of scenario $k$.
%
%
%
%
%
%, and the
%amount of different items is given by $|G_\cali| =
%n_{G_\cali}$. Let $\calt$ be a collection of subsets
%(types) of $\{1,2,\dots,d\}$, where $|\calt|
%= \calo(2^d)$, which is constant since $d$ is a
%constant. Observe that $\calt$ represents the set of all
%combinations of scenarios, so for each $t \in \calt$, consider
%$G_t = \{i \in G_\cali | i \text{ is from type } t$ representing
%the subset of items that appear in exactly the same scenarios
%described by $t$, of size $|G_t| = N_t$.
%
%
%
%
%\begin{lemma}
%    $\bar G^1_t \parallel \bar G^2_t \parallel \dots \parallel \bar G^{m_t}_t \preccurlyeq G_t$
%\end{lemma}
%\begin{proof}
%    For each item $i \in \bar G^e_t$, for $e \in \{1,2,\dots,m_t\}$, it is true that $s_i \leq s_j$ for all $j \in G^{e-1}_t$. In other words, $i$ is always ``covered" in size by some item from the previous part.
%\end{proof}
%
%
%
%Consider
%$$G^0_\cali = (G^0_{t_1} \parallel  G^0_{t_2} \parallel \dots \parallel G^{0}_{t_{|\calt|}}),$$ and
%$$G^{1,\dots,t_{|\calt|}}_\cali = (G^1_{t_1} \parallel  G^1_{t_2} \parallel \dots \parallel G^{1}_{t_{|\calt|}}) \parallel \dots \parallel  (G^{m_{t_1}}_{t_1} \parallel  G^{m_{t_2}}_{t_2} \parallel \dots \parallel G^{m_{t_{|\calt|}}}_{t_{|\calt|}}).$$
%Then we can define
%$$\bar G^{1,\dots,t_{|\calt|}}_\cali = (\bar G^1_{t_1} \parallel  \bar G^1_{t_2} \parallel \dots \parallel \bar G^{1}_{t_{|\calt|}}) \parallel \dots \parallel  (\bar G^{m_{t_1}}_{t_1} \parallel  \bar G^{m_{t_2}}_{t_2} \parallel \dots \parallel \bar G^{m_{t_{|\calt|}}}_{t_{|\calt|}}).$$
%
%It follows that $G_\cali = G^0_\cali \parallel G^{1,\dots,t_{|\calt|}}_\cali \preccurlyeq G^0_\cali \parallel \bar G^{1,\dots,t_{|\calt|}}_\cali$, i.e. a feasible solution for $G^0_\cali \parallel \bar G^{1,\dots,t_{|\calt|}}_\cali$ leads to a feasible solution of $G_\cali$. Thus $\opt(G_\cali) \leq \opt(G^0_\cali \parallel \bar G^{1,\dots,t_{|\calt|}}_\cali)$.
%
%
%
%
%Consider $G_\cali$ separated by type $\calt = \{t_1, t_2, \dots, t_{|\calt|}\}$. It is true that:
%\begin{align*}
%    G_\cali &= G_{t_1} \parallel G_{t_2} \parallel \dots \parallel G_{t_{|\calt|}} \\
%                  &= (G^0_{t_1} \parallel  G^1_{t_1} \parallel \dots \parallel G^{m_{t_1}}_{t_1}) \parallel (G^0_{t_2} \parallel  G^1_{t_2} \parallel \dots \parallel G^{m_{t_2}}_{t_2}) \parallel \dots \parallel  (G^{0}_{t_{|\calt|}} \parallel  G^{1}_{t_{|\calt|}} \parallel \dots \parallel G^{m_{t_{|\calt|}}}_{t_{|\calt|}}) \\
%                  &= (G^0_{t_1} \parallel  G^0_{t_2} \parallel \dots \parallel G^{0}_{t_{|\calt|}}) \parallel (G^1_{t_1} \parallel  G^1_{t_2} \parallel \dots \parallel G^{1}_{t_{|\calt|}}) \parallel \dots \parallel  (G^{m_{t_1}}_{t_1} \parallel  G^{m_{t_2}}_{t_2} \parallel \dots \parallel G^{m_{t_{|\calt|}}}_{t_{|\calt|}})
%\end{align*}
%
%Consider
%$$G^0_\cali = (G^0_{t_1} \parallel  G^0_{t_2} \parallel \dots \parallel G^{0}_{t_{|\calt|}}),$$ and
%$$G^{1,\dots,t_{|\calt|}}_\cali = (G^1_{t_1} \parallel  G^1_{t_2} \parallel \dots \parallel G^{1}_{t_{|\calt|}}) \parallel \dots \parallel  (G^{m_{t_1}}_{t_1} \parallel  G^{m_{t_2}}_{t_2} \parallel \dots \parallel G^{m_{t_{|\calt|}}}_{t_{|\calt|}}).$$
%Then we can define
%$$\bar G^{1,\dots,t_{|\calt|}}_\cali = (\bar G^1_{t_1} \parallel  \bar G^1_{t_2} \parallel \dots \parallel \bar G^{1}_{t_{|\calt|}}) \parallel \dots \parallel  (\bar G^{m_{t_1}}_{t_1} \parallel  \bar G^{m_{t_2}}_{t_2} \parallel \dots \parallel \bar G^{m_{t_{|\calt|}}}_{t_{|\calt|}}).$$
%
%It follows that $G_\cali = G^0_\cali \parallel G^{1,\dots,t_{|\calt|}}_\cali \preccurlyeq G^0_\cali \parallel \bar G^{1,\dots,t_{|\calt|}}_\cali$, i.e. a feasible solution for $G^0_\cali \parallel \bar G^{1,\dots,t_{|\calt|}}_\cali$ leads to a feasible solution of $G_\cali$. Thus $\opt(G_\cali) \leq \opt(G^0_\cali \parallel \bar G^{1,\dots,t_{|\calt|}}_\cali)$.
%
%
%
%
%    Consider $G^0_\cali = (G^0_{t_1} \parallel G^0_{t_2} \parallel \dots \parallel G^0_{t_{|\calt|}})$, with each $|G^0_{t_k}| = \tilde \eps N_{t_k}$ for $k \in \{1, 2, \dots, |\calt|\}$. Then, a feasible solution for $G^0_\cali$ requires a number of bins:
%    \begin{align*}
%        \sum_{k=1}^{|\calt|} \tilde \eps N_{t_k} &= \tilde \eps \sum_{k=1}^{|\calt|} N_{t_k} \\
%                                                         &= \tilde \eps n_{G_\cali}.
%    \end{align*}
%    Consider that a bin $b$ in the optimal solution has volume $V(b) = d$ (the capacity of the bin summed over all scenarios), then we have $V(i) \geq d_i s_i$ for $i \in \cali$ and $d_i$ being the number of scenarios in which item $i$ appears. It follows then that $V(i) \geq \eps$, thus $V(G_\cali) \geq \eps n_{G_\cali}$.
%    \begin{align*}
%        \obj(\calp(G^0_\cali)) &= \tilde \eps n_{G_\cali}
%                                            = \frac{\eps^2}{d^3} n_{G_\cali}
%                                            = \frac{\eps}{d^3}\eps n_{G_\cali} \\
%                                            &\leq \frac{\eps}{d^3} \frac{V(G_\cali)}{d} \\
%                                            &\leq \frac{\eps}{d^2} (V(L_1) + V(L_2) + \dots + V(L_d) \\
%                                            &\leq \frac{\eps d}{d^2} \max_{r=1,\dots,d} V(L_r) \\
%                                            &\leq \eps \big (\frac{\max_{r=1,\dots,d} V(L_r)}{d}\big ) \\
%                                            &\leq \eps \opt(G_\cali),
%    \end{align*}
%    where $L_1, L_2, \dots, L_d$ represents the items in scenarios $1$ to $d$ respectively, thus each item appear in at most $d$ scenarios.


\section{OLD APTAS}

Consider an instance $\cali = G_\cali \cup P_\cali$ of the BPS, where $G_\cali$
is the set of items greater than~$\eps$ and $P_\cali$ is the set of items
smaller than or equal to~$\eps$. Let $\calp^*(\cali)$ be an optimal packing
for~$\cali$ of value $\obj(\calp^*(\cali))$.

Perform a transformation of items in $G_\cali$ to obtain $G_\cali^0 \parallel
G_\cali^{1,\dots,|\calt|}$. Then obtain $G_\cali^0~\parallel~\bar
G_\cali^{1,\dots,|\calt|}$ through $\phi$ mapping of
$G_\cali^{1,\dots,|\calt|}$.

Consider $\calp^1(\cali)$ obtained from $\calp^*(\cali)$ by removing the items
from $G_\cali^0$ from the solution and packing each item $i \in G_\cali^0$ in a
single bin by themselves. Notice that it has been proven that
$\obj(\calp^1(\cali)) \leq (1+\eps) \opt(\cali)$
(Lemma~\ref{lemma:large_items}).

Consider $\calp^2(\cali)$ as the solution obtained by applying $\phi$-mapping into $\calp^1(\cali)$. Notice that since the items in $G_\cali^0$ have been removed from $\calp^1(\cali)$, then the items from $G_\cali^1$ become $G_\cali^0$, the items from $G_\cali^2$ become $G_\cali^1$ and so on. It is important to remark that the number of bins in $G_\cali^0$ does not change, and that $\obj(\calp^2(\cali)) \leq \obj(\calp^1(\cali))$.

Consider $\calp^3(\cali)$ a packing of $G_\cali^0 \parallel \bar G_\cali^{1,\dots,|\calt|} \parallel P_\cali$, with $P_\cali$ being the items from $\cali$ with size smaller than or equal to $\eps$. In this case, we have $\obj(\calp^3) = \obj(\calp^2)$.

Consider also $\calp^4$ obtained from $\calp^3$ by for each $t \in \calt$ and for each bin $b$ de $\calp^3$ doing:
\begin{itemize}
    \item $I_t = \{i \in \cali \mid $ $i$ is in bin $b$ and is of type $t$ $\}$;
    \item $S_t = \sum_{i \in \cali_t} s_i$;
    \item Exchange $\cali_t$ for $\lceil s_t / \hat \eps \rceil$ copies an item of size $\hat \eps$ and type $t$, possibly increasing the size of the bin in $\hat \eps$ by item, all the way to $1+ 2^d \hat \eps$ (since there are at most $2^d = |\calt|$ types of items)
\end{itemize}

% in this paragraph, I used P*_I instead of G*_kt since, as I understood, we were referring to the small items.
Regarding $\calp^4(\cali)$, it can be noticed that each bin was increased in at most $2^d \hat \eps$. Also, the packing of $G_\cali^0 \parallel \bar G_\cali^{1,\dots,|\calt|} \parallel P^*_{\cali_t}$ in which $P^*_{\cali_t}$ are the groups obtained from $P_\cali$ by transforming the small items in items $i_t$ of size $\hat \eps$ and demand $d_{i_t}$. It follows that $|P_{\cali_t}| \leq |P^*_{\cali_t}|$

With this, we have that $\calp^4(\cali)$ induces a packing $\bar H$ of $\bar G^{1,\dots,|\calt|} \parallel P_{\cali_t}$.

% I don't know what we were referring to as B_u
\begin{lemma}\label{lemma:small_items1}
    $\bar H$ is a feasible solution in $\bar B_u$, then $\obj(\bar H) \leq \obj(\calp^*(\cali)) = \opt(\cali)$ and $|G^0_\cali| \leq \eps \obj(\calp^*(\cali)) = \eps \opt(\cali)$.
\end{lemma}

\begin{lemma} \label{lemma:small_items2}
    There is a solution $H$ of $G^{1,\dots,|\calt|}_\cali \parallel P_\cali$ in bins of size $1$ and cost at most $(1+\eps)\opt(H^*) + 1$, where $H^*$ is an optimal solution in $\bar B_u$.
\end{lemma}

\begin{proof}
    For each $\bar j \in \bar G^{1,\dots,|\calt|}_\cali$, exchange $\bar j$ for its respective $j \in G^{1,\dots,|\calt|}_\cali$, where $\phi^{-1}(\bar j) = j$. For each type $t \in \calt$, pack the items of $G_{\cali_t}$ in some bin. It is important to remind that items of same size $\hat \eps$ are grouped by type. The items from group $G_{\cali_t}$ in the region formed by the grouping of items of size $\hat \eps$. We refer to this grouping as a \textit{slice}.
    % this part gets a little confusing with the concept of slices
    For each bin and each type, pack $\eps G_{\cali_t}$ in a way that they cover all items of size $\hat \eps$ for that type, eventually having some item violating the size of the slice, but not more than one slice. Items can be moved inside a slice so that the item that violates it becomes fully covered by the slice. The capacity of the bin may be violated.

    \begin{fact}
        All items of $P_\cali$ are allocated to some bin.
    \end{fact}

    \begin{fact}
        The sum of all the sizes of items that violate the bin size is $2 \dot 2^d \hat \eps = \bar \eps$, since there are at most $2^d$ slices for all $d$ types and the last slice of each type can have one exceeding item.
    \end{fact}

    The small items packed after $1$ and before $2 \bar \eps$ are organized in slices such that the total size of the slice is at most $|H^*|2 \bar \eps$. Assuming that $1 / 2 \bar \eps$ is integer, then all slices can be grouped in $\lceil |H^*| / \frac{1}{2 \bar \eps} \rceil \leq 2 \bar \eps |H^*| + 1$. Since $|H^*|/2 \leq \obj(H^*)$, it follows that the number of bins created is $2 \bar \eps 2 (\frac{|H^*|}{2}) + 1 \leq 4 \bar \eps \obj(H^*) + 1$. Thus, considering $\obj(\calp(G^{1,\dots,|\calt|}) \leq \obj(H^*)$, it follows that $\obj(\calp(G^{1,\dots,|\calt|} \parallel P_\cali) \leq \obj(H^*) + \eps_0 \obj(H^*) + 1 = (1+\eps_0) \obj(H^*) + 1$.\qed
\end{proof}

\begin{theorem}
    There is an polynomial time algorithm such that the value of its solution is at most $(1+\eps)\opt(\cali) + 1$ for the BPS.
\end{theorem}

\begin{proof}
    By Lemma~\ref{lemma:small_items1}, we have that $\obj \calp(G^0) \leq \eps \opt(\cali)$, and by Lemma~\ref{lemma:small_items2} we have that $\obj(\calp(G^{1,\dots,|\calt} \parallel P_\cali)) \leq (1+\eps_0) \opt(\cali) + 1$. Thus it follows that $\obj(\calp(G^0 \parallel G^{1,\dots,|\calt} \parallel P_\cali)) \leq (1+\eps) \opt(\cali) + 1.$\qed
\end{proof}

